Stationary time-vertex signal processing

This paper considers regression tasks involving high-dimensional multivariate processes whose structure is dependent on some {known} graph topology. We put forth a new definition of time-vertex wide-sense stationarity, or joint stationarity for short, that goes beyond product graphs. Joint stationarity helps by reducing the estimation variance and recovery complexity. In particular, for any jointly stationary process (a) one reliably learns the covariance structure from as little as a single realization of the process, and (b) solves MMSE recovery problems, such as interpolation and denoising, in computational time nearly linear on the number of edges and timesteps. Experiments with three datasets suggest that joint stationarity can yield accuracy improvements in the recovery of high-dimensional processes evolving over a graph, even when the latter is only approximately known, or the process is not strictly stationary.

==> macros.tex <==

% TEXT SHORTHANDS
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\renewcommand{\etal}{et al.\xspace}
\renewcommand{\paragraph}[1]{\vspace{3mm}\noindent\textbf{#1}}
\newcommand{\todo}[1]{{\color{red}{\textbf{todo:} #1}}}
\newcommand{\shorten}[2]{#2}

% MATH SHORTHANDS
\renewcommand{\b}[1]{{\bm{#1}}}   % bold symbol

% MATH SYMBOLS
\newcommand{\1}{\b{1}}              % all-ones vector
\newcommand{\0}{\b{0}}              % all-zero vector
\newcommand{\x}{\b{x}}
\newcommand{\s}{\b{s}}
\newcommand{\h}{\b{h}}
\newcommand{\w}{\b{w}}
\newcommand{\y}{\b{y}}
\renewcommand{\u}{\b{u}}
\renewcommand{\v}{\b{v}}
\newcommand{\e}{\b{e}}
\newcommand{\eps}{\bm{\varepsilon}} 
\renewcommand{\L}{\b{L}}            % The combinatorial Laplacian
\newcommand{\U}{\b{U}}              % an eigenvector matrix
\newcommand{\bSigma}{\b{\Sigma}}    % a covariance matrix
\newcommand{\bLambda}{\b{\Lambda}}  % a diagonal matrix of eigenvalues
\newcommand{\bOmega}{\b{\Omega}}  % a diagonal matrix of eigenvalues
\newcommand{\bGamma}{\b{\Gamma}}  % a diagonal matrix of eigenvalues
\newcommand{\blambda}{\b{\lambda}}  % a vector of eigenvalues
\newcommand{\bomega}{\b{\omega}}  % a vector of eigenvalues
\newcommand{\M}{{\b{M}}}
\renewcommand{\H}{{\b{H}}}
\newcommand{\I}{\b{I}}
\newcommand{\A}{\b{A}}
\newcommand{\B}{\b{B}}
\newcommand{\X}{\b{X}}
\newcommand{\Y}{\b{Y}}
\newcommand{\V}{\b{V}}              % right singular vectors
\newcommand{\D}{\b{D}}              % singular values
\newcommand{\W}{\b{W}}              % the adjacency matrix
\renewcommand{\O}{O}              

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{#2}}%

% Laplacian matrices
\newcommand{\LG}{\L_{\hspace{-1px}G}}              % Graph
\newcommand{\LJ}{\L_{\hspace{-1px}J}}              % Joint
\newcommand{\LT}{\L_{\hspace{-1px}T}}              % TIme

% Localization operators
\newcommand{\TG}[2]{{\mathcal{T}_{#2}^{\hspace{1px}G}} #1 \hspace{0.2mm}}              % Graph
\newcommand{\TGL}[2]{{\mathcal{T}_{#2}^{\hspace{1px}G}} \left(#1\right) }              % Graph
\newcommand{\TJ}[2]{{\mathcal{T}_{#2}^{\hspace{1px}J}} \hspace{0.5mm} #1 \hspace{0.2mm}}              % Joint
\newcommand{\TT}[2]{{\mathcal{T}_{#2}^{\hspace{1px}T}} #1 \hspace{0.2mm}}              % Time

% Fourier matrices
\newcommand{\UG}{\U_{\hspace{-1px}G}}              % Graph
\newcommand{\UJ}{\U_{\hspace{-1px}J}}              % Joint
\newcommand{\UT}{\U_{\hspace{-1px}T}}              % TIme

% MATH TRANSFORMS
\newcommand{\GFT}[1]{\textrm{GFT}\hspace{-.0mm}\{#1\}}
\newcommand{\IGFT}[1]{\textrm{GFT}^{\hspace{0.2mm}\Scale[0.7]{-1}}\hspace{-.0mm}\{#1\}}
\newcommand{\DFT}[1]{\textrm{DFT}\hspace{-.0mm}\{#1\}}
\newcommand{\JFT}[1]{\textrm{JFT}\hspace{-.0mm}\{#1\}}
\newcommand{\IJFT}[1]{\textrm{JFT}^{\hspace{0.2mm}\Scale[0.7]{-1}}\hspace{-0.0mm}\{#1\}}
\newcommand{\STFT}[1]{\textrm{STFT}\hspace{-.0mm}\{#1\}}

% Sets of numbers
\newcommand{\Rbb}{\mathbb{R}} 
\newcommand{\Cbb}{\mathbb{C}}

% MATH OPERATORS
\newcommand{\E}[1]{\mathbf{E}\hspace{-.3mm}\left[#1\right]}        % the expectation operator
\newcommand{\Es}[1]{\tilde{\mathbf{E}}\hspace{-.3mm}\left[#1\right]}        % the sample average operator
\newcommand{\var}[1]{\mathbf{Var}\hspace{-.3mm}\left[#1\right]}        % the expectation operator
\renewcommand{\P}[1]{\mathbb{P}\left[#1\right]}        % the probability operator
\renewcommand{\mod}[2]{\textrm{mod}\hspace{-.5mm}\left(#1,#2\right)}           % the modulo operation 
\renewcommand{\vec}[1]{\textrm{vec}\hspace{-.5mm}\left(#1\right)}           % the vectorization operator
\newcommand{\mat}[1]{\textrm{mat}\hspace{-.5mm}\left(#1\right)}           % the matrization operator
\newcommand{\diag}[1]{\textrm{diag}\hspace{-.5mm}\left(#1\right)}           % defining a diagonal matrix from vector
\newcommand{\trace}[1]{\textrm{tr}\hspace{-.5mm}\left(#1\right)}            % the trace operator
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}        % a matrix norm
\newcommand{\transpose}{\intercal}                      % the  transpose
\newcommand{\hermitian}{*}                      % the  transpose
\newcommand{\delequal}{\overset{\Delta}{=}} % define equal

% Theorem enviroments
\newtheorem{theorem}{Theorem} \newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition} \newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark} \newtheorem{corollary}{Corollary}
\newtheorem{property}{Property} 
\newtheorem{example}{Example}
\newtheorem{featuredtheorem}{Featured Theorem}



\newcommand{\nati}[1]{{\color[rgb]{.1,.7,.1}{#1}}}
\newcommand{\andreas}[1]{{\color[rgb]{.1,.1,.9}{#1}}}
